Composing Option Sequences by Adaptation: Initial Results

Robot manipulation in real-world settings often requires adapting the robot's behavior to the current situation, such as by changing the sequences in which policies execute to achieve the desired task. Problematically, however, we show that composing a novel sequence of five deep RL options to perform a pick-and-place task is unlikely to successfully complete, even if their initiation and termination conditions align. We propose a framework to determine whether sequences will succeed a priori, and examine three approaches that adapt options to sequence successfully if they will not. Crucially, our adaptation methods consider the actual subset of points that the option is trained from or where it ends: (1) trains the second option to start where the first ends; (2) trains the first option to reach the centroid of where the second starts; and (3) trains the first option to reach the median of where the second starts. Our results show that our framework and adaptation methods have promise in adapting options to work in novel sequences.

==> backup_files/backup.tex <==
\iffalse{
Abstract from Friday at 1:08PM:
For a robotics manipulation task, composing a sequence of five Deep RL options for goal-conditioned RL does not result in a sequence that can complete the overall task when the options are trained independently.  We examine three approaches that train pairs of options to sequence successfully by considering the actual subset of points that the option is trained from or where it ends: 1) trains the first option to reach the centroid of the second option's starting set; 2) trains the first option using the median of the second option; and 3) trains them in tandem.  Our results show that the tandem training performs best, suggesting that adapting RL options to work in sequence, at least for this manipulation task, will often mean retraining the option but also that the training needs to consider the subset of states where the options are trained from or where they reach.  

Intro at Friday at 1:08PM:
One way to reduce the sample complexity of reinforcement learning is by using frameworks with temporally extended actions such as the Options Framework \citet{SUTTON1999181} 
However, the options framework and derivatives (e.g., \cite{bacon2016optioncritic, composable_parameterized_skills, symbolicRepParamSkills, fromSkillsToSymbols, skill_discovery, bagaria_21, Patra_Cavolowsky_Kulaksizoglu_Li_Hiatt_Roberts_Nau_2022}) often assume that options can be sequenced to complete tasks. In practice, however, options that are not trained together; i.e., they are independently trained, may not execute successfully when sequenced to complete tasks as noted by \citet{logical_options_framework} and \citet{kumar2024practice}.

To illustrate this, we train five independent options that, together, perform a pick-and-place task (Figure~\ref{fig:pickandplace}).  Each pair in this sequence has overlapping termination (TERM) and initiation (INIT) conditions, so they should, in theory, execute successfully to complete the task.  Surprisingly, however, we demonstrate that these five options fail to execute the task to completion when trained independently.  We provide evidence that the key reason for this failure has to do with a mismatch between where the first option ends and the next option begins; in other words, we can not assume successful execution of sequenced options just because they are connected. The successful execution of connected options, in seems, has more to do with how these options are \emph{trained} than how they are XXXXX.

% the failure has to do with how these skills are \emph{trained}. 

In this paper, we provide a formal analysis of why the distinction between overlapping conditions and overlapping training is crucial to successfully sequencing options (Section~\ref{sec: composablesec}). We then introduce three methods to adapt independent options so that their performance when connected together improves (Section~\ref{sec:adaptationsection}). Next, we introduce metrics for measuring how closely two options can cooperate, and evaluate the adaptation methods (Section~\ref{sec:results}). Our results show that adapting connected options so that the are more tightly coupled (i.e., dependent) provides the greatest benefit.
} %\iffalse

% Talk about the need for complex manipulation behavior of robots in order to solve the necessary daily active tasks. Then discuss what is necessary to provide robots with these behaviors and then talk about how current abtraction methods with assumed composability won't allow for flexible changes in skills and then discuss how my work is aimed to addrees how to learn independent skills that can be  connected by a planner and evaluated to see if they are compatible and adapted when they are fouind not to be compatible.
\iffalse 
The number of households with the head of the household being 80 and over is projected to increase to nearly 17 million in the U.S. by 2040 \cite{HousingStudy}. According to the Housing Studies of Harvard University 2023 report \cite{HousingStudy}, these households have a higher likelihood to report difficulties with self-care, independent living, and mobility, which indicates that there will be a high demand for caregivers to help these individuals in the coming future. In a recent survey of 144 nursing home providers conducted by the American Health Care Association, seven out of ten nursing homes reported that their health care staffing levels are still lower than the levels they had before the COVID pandemic, and 96\% reported having difficulties in recruiting new staff \cite{HealthCareSurvey}. Therefore to meet this health care demand, domestic service robots have been proposed as a possible solution \cite{sawik_robots_2023}. 

Some of the activities of daily living that domestic service robots could help out with are transportation and shopping, meal preparation, housecleaning and home maintenance, and managing medications, among others \cite{ADLs}. At least three of these activities (meal preparation, housecleaning, and home maintenance) require the robot to posses complex and generalizable motor skills. A possible housecleaning task could be putting away clean cups into a cabinet. This manipulation task can be decomposed into a sequence of motor skills for a robotic arm to perform. According to \cite{yadav_reflecting_2023}, motor skills for humans are made up of simpler motor primitives. Motor primitives can be thought of as fundamental building blocks for constructing motion \cite{giszter_motor_2015}. Even though motor primitives are simplistic by nature, humans possess the ability to complete complex manipulation tasks by learning, adapting, and composing motor primitives into a wide variety of motor skills \cite{yadav_reflecting_2023}.  If robots possessed this ability, then they could complete complex manipulation tasks that will be required of them as part of their service duties. 

For these robots to provide help autonomously, they will be faced with having to take actions in unstructured environments. To deal with acting in unstructured environments, reinforcement learning and then later deep reinforcement learning are two learning methods which through interactions with the environment can build a policy that will select actions based on the current state of the environment. In theory, if all possible interactions with the environment were learned, then the policy would be able to choose the correct action no matter the current state of the environment. In practice, deep reinforcement learning methods have been shown to have good performance in robotic domains \citet{learningtowalk}, but their performance suffers when interaction time with the environment is low \citet{haarnoja2018composable}. 

High sample complexity is necessary for many deep reinforcement learning methods to perform well which is not always possible. 

This is due to the fact that during training these skills are combined to figure out which combinations will solve the high level task which means that the learned skills become dependent on one another for execution.

\fi %end iffalse

%, which we call goal skills, which are variants of options, are trained independently but composed to perform an example pick and place manipulation task. The importance of independent skills is derived from the need to deal with robotic hardware that has pretrained skills, skills learned from demonstration or more simply the need to mix new and previously trained skills in order to accomplish complex behaviors. To complete complex manipulation tasks that are decomposed into sequences of skills, a combination of a temporal abstraction methods and the ability to train and compose independent skills is necessary. 
%The definition of goal skills and how they were trained is presented in Section \ref{learningIndependentSkills}. In Section \ref{sec: composablesec}, we verify and validate that an ordered sequence of independent goal skills is composable, and therefore can successfully execute the pick and place task in simulation.  If this sequence of goal skills can not execute the task successfully due to certain goal skills in the sequence not being composable then it is necessary to adapt those skills to be composable rather than retraining the full sequence of goal skills. Three different adaptation methods are presented in Section \ref{sec:adaptationsection}. Lastly, the rate of successful task completion was measured given sequences of goal skills that were adapted by one of the the three adaptation methods in order to compare the methods and future directions for adaptation of goal skills are discussed. 

% Composability of actions or skills (extended actions) is the key to the reuse of learned knowledge \citet{mendez2023reuse}. If skills are composable, it is possible to learn in simpler environments and compose multiple skills to achieve more complex tasks. Further, composable skills can be arranged in novel ways thereby transferring learned knowledge to complete novel tasks which enables positive transfer \citet{mendez2023reuse}.  

\iffalse

\citet{SUTTON1999181} introduced the Options Framework where an option is made up of an initiation set $I \subseteq S$, a policy $\pi:S \times A \rightarrow [0,1]$, and termination condition $\beta:S^+ \rightarrow [0,1]$ where $S$ is the perceived states of the environment and $S^+$ is the set of perceived states ($S$) plus the terminal state of an episode of a Markovian task. In \citet{Patra_Cavolowsky_Kulaksizoglu_Li_Hiatt_Roberts_Nau_2022}, the authors discussed that goals are symbolic states or sets of states that can be achieved by an agent, and skills are policies which are mappings of states to actions. A goal skill is the link between goals and skills \cite{Patra_Cavolowsky_Kulaksizoglu_Li_Hiatt_Roberts_Nau_2022}. A goal skill is defined by \citet{Patra_Cavolowsky_Kulaksizoglu_Li_Hiatt_Roberts_Nau_2022}:

\begin{definition}[Goal Skill]\label{def:goal_skill}
    A \emph{goal skill} $g_\pi = (head, \hat{g}, \hat{\pi}, \mathscr{C})$ is a tuple where \emph{head} includes the \emph{name} and \emph{parameters} of the goal skill, $\hat{g}$ contains the goal information the skill is meant to achieve, $\hat{\pi}$ is the goal-specific policy, and $\mathscr{C}$ is a non-empty set of conditions. 
\end{definition}

$\mathscr{C}$ is partitioned into $\{\mathscr{C}_{start}, \mathscr{C}_{during}, \mathscr{C}_{end}\}$ which are conditions that define sets of states. Formally, 

\begin{definition}[Initialization Conditions] 
    $\mathscr{C}_{start}$ is the set of conditions that define the set of states (Initiation Set, $I \subseteq S$) from which the goal skill can be executed.
\end{definition}

\begin{definition}[Maintenance Conditions]
    $\mathscr{C}_{during}$ is a set of conditions that must be satisfied during execution of the goal skill. 
\end{definition}

\begin{definition}[Termination Conditions]
    $\mathscr{C}_{end}$ is the set of conditions that define the set of states (Termination set, $T \subseteq S$)  where the termination conditions are satisfied, and the goal skill execution 
    terminates.
\end{definition}

The initiation set, $I$, and the termination conditions, $\mathscr{C}_{end}$, are similar to the initiation set and termination conditions of an option from the Options Framework \cite{SUTTON1999181}. A goal skill differs from an option due to the maintenance conditions which enables better control over the behavior of the goal skill policy.
\fi

\iffalse 
\subsection{Training Independent Goal Skills}

For this work, a pick and place task was manually decomposed into an ordered sequence of five goal skills. This simplified the problem to defining those five goal skills and setting up independent goal skill training. As well as, evaluating the composability of the ordered sequence of independent goal skills and finding methods for adapting goal skills to be composable when they were found to be non-composable. The decomposition of a pick and place task is shown in Figure \ref{fig:pickandplace}. The five goal skills that we use in sequence for a pick and place task are: $Reach(item) \rightarrow Grasp(item) \rightarrow Lift(item, target) \rightarrow Carry(item, target) \rightarrow Place(item, target)$. The goal skill definitions that include information about the initiation, maintenance, and termination conditions for each goal skill are in Appendix \ref{sec:appendix}. 

A robotic environment for the pick and place task was developed to be a part of robosuite, a simulation framework powered by MuJoCo physics engine for robotic learning \cite{robosuite2020}. Robosuite has suite of robotic arms, controllers, objects and sensors. Figure \ref{fig:kinova3sim} shows the pick and place environment that was used for training each goal skill. Kinova Gen3 \cite{kinovagen3} robotic arm pictured in Figure \ref{fig:kinova3sim} is a seven degree of freedom robotic arm.  

\fi 


% Defining connected and composable goal skills section
\iffalse

For sequences of goal skills to be feasible and to execute successfully, we found in practice that goal skills need to be connected and composable. These two concepts relate the \emph{training}.


Connected goal skills are connected when the termination set of a goal skill is a subset of the initiation set of the succeeding goal skill in a sequence. Goal skills are composable when they are connected and their policies can be executed successfully one after another to termination.  However, before we more formally define connected and composable goal skills, it is necessary to define two more sets of states which are subsets of the Initialization and Termination sets of a goal skill. 

\begin{definition}[Origin Set] \label{originset}
The \emph{origin set}, $\mathscr{O}$, is the set of states in which the policy actually initiates from, $\mathscr{O} \subseteq I$.
\end{definition}

\begin{definition}[Result Set] \label{resultset}
The \emph{result set}, $\mathscr{R}$, is the set of states in which the policy actually triggers the termination conditions of $\mathscr{C}_{end}$ where $\mathscr{R} \subseteq T$.
\end{definition}

Given Definitions \ref{originset} and \ref{resultset} and two goal skills, $g_{\pi_{i}}$ and $g_{\pi_{j}}$, where the execution of $g_{\pi_{i}}$ precedes that of $g_{\pi_{j}}$:

\begin{definition}[Connected Goal Skills] \label{Connectedgoalskills}
Goal skills, $g_{\pi_{i}}$ and $g_{\pi_{j}}$, are connected if $T_i \subseteq I_j$.
\end{definition}

\begin{definition}[Composable Goal Skills] \label{Composablegoalskills}
Goal skills, $g_{\pi_{i}}$ and $g_{\pi_{j}}$, are composable if goal skills, $g_{\pi_{i}}$ and $g_{\pi_{j}}$, are connected and $\mathscr{R}_{i} \subseteq \mathscr{O}_{j}$.
\end{definition}
\fi 


% Along with coming up with a method to compose independent skills, there is a need to verify and validate that skills can be connected and are composable. Reward machines were created as a way to use linear temporal logic (LTL) and b\"{u}chi automata to guide an agent to learn various skills \citet{IcarteRLLTL2018}. Further, reward machines have shown that they learn an optimal plan of sub-tasks(skills), but these skills are not reusable or composable components outside of the plans that have been seen in the training set. The use of LTL and automata was to reduce the need of reward function shaping or creation, but the authors did not verify the skills connectivity using formal methods. For the Logical Options Framework in \citet{logical_options_framework}, the authors state that their plans (sequences of skills) are satisfying, optimal, and composable, but the learned skills still require retraining to be composable to unseen tasks \citet{logical_options_framework}. While their retraining methods are low in number of training samples, this is entirely dependent on the length and variance of the new unseen task from the learned tasks. The number of training samples would increase with the increase in difficulty and variation of the new unseen tasks versus the tasks that have been seen during training. For this work, it is hypothesized that possessing a method for adapting independent skills that then would be composable would require less overall training as compared to retraining entire chains or sequences of skills. 

% In \citet{logical_options_framework}, LTL and b\"{u}chi automata are also used to ensure liveness and safety contraints, but timing constraints can not be verified which is why this work will propose to use metric interval temporal logic (MITL) \citet{mitlAlur1996} and model checking software such as UPPAAL \citet{uppaal} to verify timing constraints of plans which is necessary for Real-Time systems like robotic systems. For validation, methods will be created to use data derived from simulation to validate already verified plans. The combination of temporal abstraction methods and curricula used for learning, the ability to verify and validate sequences of those temporally extended actions, and adaptation methods when sequences are found invalid will lead to plans that can be executed on robotic hardware and the tools to better monitor that execution.

Since the place task was manually decomposed, the ordered sequence of goal skills were authored to be connected. Therefore, for each goal skill in the place task, Definition \ref{Connectedgoalskills} was satisfied. However, since the goal skills are independent of one another, this sequence of goal skills still needs to be checked to see if it is composable. 

Compatibility is a measure of the performance success of connected goal skills. For instance, if the last goal skill in a connected sequence of goal skills is successful every time this sequence of skills was executed, this sequence would be measured to be 100\% compatible and deemed composable. Any compatibility score less than 100\% indicates that goal skills are not composable.

The performance success of connected goal skills is measured by executi rollouts (executions) of the connected goal skills in simulation. A successful completion of execution is when the last goal skill in the sequence of connected goal skills terminates successfully. Compatibility is measured by dividing the number of successful completions out of the total number of rollouts and multiplying this number by 100 to get the percentage of success.


\iffalse \frommak{no longer needed, given the above definition..}
\begin{definition}[Connected Options] \label{Connectedgoalskills}
Two options \optioni and \optionj are connected if $\termset{i} \subseteq \initset{j}$.
\end{definition}
\fi 

For these rollouts, the agent starts in a state inside of the set, $\mathscr{O}_l$. The agent will then follow the policy $\pi_l$ until successful termination in $\mathscr{R}_l$ which at that point the start state will be saved to a file. These rollouts are performed until an adequate number of samples are collected which in practice has been around 1000 samples. 

The time of sample collection depends on the number of timesteps needed to reach goal termination per episode which on average for the goal skills that have been tested has been roughly 8 timesteps or 0.78 seconds per episode.  


% discusing RM - centroid method downside
RM-Centroid was the first attempt at moving the result set of goal skills to be a subset of the origin set of the succeeding goal skill, but it did not achieve the same level of performance for the all of the goal skills that were being tested. One hypothesis is that the selecting a sample that is close to the centroid of the origin set might result in a sample that does not have a lot of samples nearby or is not locally dense. This could affect the composability of the goal skills. Based on RM-Centroid which is able to move the result set of a goal skill, if the terminal states of the new result set as seen in blue in Figure \ref{fig:liftAdaptedDep} are in an area of the origin set which is not locally dense then there could still be issues of ending in states that lie outside of the policy distribution for the succeeding goal skill.

\iffalse
The independent goal skills are not compatible for any sequence of connected goal skills, except between the grasp and lift goal skills which is why RM-Centroid and RM-Density were not applied to the grasp goal skill. As discussed in Section \ref{sec:dependentmethod}, it is necessary to apply the dependent method to every goal skill since this method creates new policies with different results sets. This is also the reason why this method works so well across all goal skills because every goal skill is being adapted to work with the next goal skill in the sequence. However, RM-Centroid and RM-Density both perform as well or better than the dependent method except for the sequences involving carry and place goal skills. Due to this performance drop, the final connected sequence of all of the goal skills scored very low for compatibility when using the result methods. The reason for this failure to the adaptation of this pair of goal skills is still being investigated.
\fi 

\iffalse

The objective of using RM-Centroid or RM-Density is to find methods that reduce the amount of retraining necessary as compared with the dependent method. In order to test this objective, the total number of training steps taken until policy convergence is shown in the bar chart of Figure \ref{fig:trainingsamples}. The number of training samples are higher for the result methods versus the dependent method which is opposite to what was hypothesized. However, this sequence of skills was small and the skills themselves did not take many samples to train independently, so it follows that the dependent method would take a similar amount of time to retrain each goal skill since there was no reward structure changes implemented for that method as done for the RMs. This does not indicate that this will apply for any and all combination of future goal skills, so there needs to be continued investigation into enhancing the dependent result methods by increasing the speed of their adaptation of skills to be compatible.

%brought down from dependent method section do not need to use 
One downside to this method is that this method needs to be applied to every option in the sequence because it creates a problem when applied to non-composable options that have at least one composable option following the adapted option as shown in Figure \ref{fig:incompatiblemiddle}. A new policy is created while expanding origin set \originset{k} which results in the creation of a new result set, $\resultset{k}'$ which is not guaranteed to satisfy $\mathscr{R'}_k \subseteq \mathscr{O}_l$. Therefore, if this dependent method was used for adaptation, it can only be applied to the incompatible skills at the end of a sequence of connected goal skills or will have to applied to every goal skill in the sequence. It could be reasonable to apply this method to shorter sequences, but the total retraining time would depend on how long the sequence of goal skills end up being.  
\fi

\iffalse
\frommak{I probably wrote this... sorry.  It's too early in the paper to give anything more than the gist, especially since we go into the details later.  So I just summarized it and removed the detail.}
To understand why, consider a pair of options $o_i$ and $o_j$, where the INIT($o_j$) is equal to TERM($o_i$). Every option will have a policy, a mapping of states to actions, that will execute if the initiation conditions of the option are satisfied and terminate if the termination conditions of the option are satisfied. Since the conditions for the INIT($o_j$) is equal to TERM($o_i$) for this simplest case, in theory, the policy, $\pi_i$, should terminate with a given probability in a state that satisfies the initiation conditions for INIT($o_j$). In practice, the independent policy trained for $o_j$ could be trained from any set of states that satisfies the INIT($o_j$). Therefore, it is not guaranteed that the terminal state of the policy, $\pi_i$, will be inside of the set of states that $o_j$ was trained from even when this terminal state satisfies the conditions of INIT($o_j$).
\fi 



\iffalse
Consider Figure \ref{fig:incompatibleend}, which plots non-composable options at the end of a sequence of composable options. Even though the sequence of options is connected, the result set, $R_j$, is not a subset of the origin set, $O_k$, which indicates that these two options are not composable. Before we can test how the origin and result set overlap affects the performance of connected options, we first need methods for adapting these origin and results sets of independently trained options. Therefore, we came up with three methods that either modify the origin or result set which we called the Origin Method, the Result Method - Centroid (RM-Centroid), and the Result Method - Density (RM-Density). 
\fi


\iffalse
We also plan to study more complex manipulation behaviors and use methods like $GTPyhop^2$ \cite{nau2021gtpyhop} to recursively decompose robotic manipulation tasks into ordered sequences of options instead of manual decomposition. This would help further test our adaptation methods to longer sequences of options.  
\fi 

% \frommak{some kind of problem here with grammar}
% , adaptation and optimality of the learned chains are still areas of focus for their works. For instance, \citet{bagaria_robust_composable_skills, bagaria_Neurips23} focused on improving how the initiation sets of skills (set of states where policies can be executed) are created in order to have a sequence of skills behave more optimally \citet{bagaria_robust_composable_skills, bagaria_Neurips23}. \citet{abbatematteo2024composable} compose manipulation skills through the use of a motion planner which makes sense to connect two states by the means of a motion plan but could result in unwanted behavior in the hand-off between skills. Further, most motion planning algorithms require static environments which indicates that the end effector needs to stop moving between skills when using a motion planner to compose skills together.

% %%%%% DISCUSS REWARD MACHINES METHODS AND LOGICAL OPTIONS PAPER HERE ESPECIALLY SINCE LOGICAL OPTIONS MAKES CLAIMS ON SATISFYING, OPTIMAL, AND COMPOSABLE PLANS. Arguement to their method is they are not flexible to mixing independently learned policies. 
